Self-Adversarial Learning with Comparative Discrimination for Text Generation

Conventional Generative Adversarial Networks (GANs) for text generation tend to have issues of reward sparsity and mode collapse that affect the quality and diversity of generated samples. To address the issues, we propose a novel self-adversarial learning (SAL) paradigm for improving GANs' performance in text generation. In contrast to standard GANs that use a binary classifier as its discriminator to predict whether a sample is real or generated, SAL employs a comparative discriminator which is a pairwise classifier for comparing the text quality between a pair of samples. During training, SAL rewards the generator when its currently generated sentence is found to be better than its previously generated samples. This self-improvement reward mechanism allows the model to receive credits more easily and avoid collapsing towards the limited number of real samples, which not only helps alleviate the reward sparsity issue but also reduces the risk of mode collapse. Experiments on text generation benchmark datasets show that our proposed approach substantially improves both the quality and the diversity, and yields more stable performance compared to the previous GANs for text generation.

==> abstract_info.tex <==
\begin{abstract}
%Generative adversarial networks (GANs) have achieved great success at generating realistic images. However, modern GAN architectures do not perform as well in text generation tasks.
The discriminator in most existing generative adversarial networks (GANs) receives a sample either generated or sampled from real data and outputs a binary score indicating the probability of the sample being real. When a good sample is generated and successfully fools the discriminator, it is indistinguishable whether the generated sample is of better or the same quality compared with real data. We propose a comparative discriminator which receives a generated sentence and a reference sentence and outputs the probability of the generated sentence is better, comparable or worse than the reference sentence. Based on the proposed comparator, we introduce a novel self-adversarial learning (SAL) paradigm where generated samples are compared with other samples generated by the generator itself instead of competing with real samples. By improving the generator in a self-play fashion, SAL is able to provide more informative and stable learning signal than standard GANs, especially when the discrepancy between generated samples and real data is large, which is often encountered in text generation tasks. The proposed comparator and SAL help alleviate issues in adversarial text generation including reward sparsity, training instability and mode collapse. Experiments on several benchmark datasets for text generation demonstrate that the proposed comparator is able to significantly and consistently outperform both standard binary discriminator and recently proposed ranker model. Furthermore, SAL yields better performance and stability compared with standard adversarial learning. We want to study it.
%the training suffers from less variance and is less sensitive to random initialization and hyperparameter choices.
\end{abstract}

\section{Introduction}

Natural Language Generation (NLG) has been widely adopted in many Natural Language Processing (NLP) applications such as machine translation~\cite{bahdanau2014neural}, dialogue generation~\cite{li2017adversarial} and image captioning~\cite{fang2015captions}. Previous approaches generally maximize the log-likelihood of ground-truth sentences. However, in theory, this approach suffers from exposure bias~\cite{bengio2015scheduled} due to the inherent discrepancy between the training stage and inference stage. That is to say, the model is trained to generate appropriate succeeding token based on ground truth prefix, which is not available during training.

%The problem of exposure bias is avoid as the generator generate tokens based on previous generated tokens in both training and inference stage.%

Recently, generative adversarial networks~\cite{goodfellow2014generative} (GANs) has been leveraged as a powerful paradigm to address the aforementioned problem. While GANs have shown some promising improvements in text generation compared with the conventional maximum likelihood estimation (MLE) method, they also suffer from several fundamental issues, including: (i) Reward sparsity, which may due to the fact that the discriminator generally learns much faster than the generator and easily recognize generated sentences as fake examples. The generator thus receives very low and non-distinctive rewards; (ii) Training instability, which exists in standard GAN training and is intensified by the policy gradient training which is known to have high variance; and (iii) Mode collapse, which is due to the intrinsic nature of GANs and makes adversarial models tend to learn limited patterns which successfully fooled the discriminator.

In this work, we first propose a comparative discriminator in the spirit of learning by comparison to relieve the reward sparsity problem. The comparator simultaneously receives a generated sentence and a reference sentence as input and outputs the comparison results indicating the probability of the first sentence is more, equally or less realistic than the reference sentence. Standard binary discriminator in GANs receives either generated or real sample and outputs a binary score indicating the probability of the received sample being real. When the a good sentence is generated, the binary discriminator would assign high probability to the sentence being real. However, it is indistinguishable whether the generated sentence is indeed better, comparable, or indeed slightly worse compared with real sentences. The comparator instead judges the quality of generated sentences by comparing them with reference sentences, thus aware of this difference and could hopefully provide more reliable and informative learning signal. Based on the proposed comparator, we next introduce a novel self-adversarial learning paradigm (SAL) which reduce training instability and mode collapse. In SAL, instead of competing with real samples, generated samples are compared with previous samples generated by the same generator and result in reward signals encoding relative improvement, which are hopefully more stable and informative. SAL helps alleviate the reward sparsity problem as comparing two generated sentences is more challenging. The comparative discriminator could not easily recognize generated sentence as fake and provide zero reward. Moreover, the relative improvement reward signal and 'tie' option of the comparator could hopefully reduce the instability of adversarial training. Finally, as the generator has to compete with itself which keeps updating, it can not merely learn limited patterns which resembles real data and keeps fooling the discriminator, thus reduce the problem of mode collapse in conventional adversarial learning.

Our contributions are three-fold: (i) We propose a comparative discriminator which evaluate the quality of generated sample by pairwise comparison. (ii) We introduce a self-adversarial learning paradigm where generator improves by making relative progress.  (iii) We evaluate our model comprehensively on text generation benchmark platform~\cite{zhu2018texygen}. The comparator consistently and significantly outperforms both binary discriminator and recently proposed ranker model~\cite{lin2017adversarial}. Self-adversarial learning with the comparator further improves both the performance and training stability. 
%Moreover, simply combining standard adversarial learning and SAL yields incremental improvements.

\begin{figure}
    \centering
    \includegraphics[width=10cm]{SAL.pdf}
    \caption{Illustration of proposed comparative discriminator and self-adversarial learning paradigm. }
    \label{fig:my_label}
\end{figure}

==> intro_bakup.tex <==
\section{Introduction}
%Natural Language Generation (NLG) has been widely adopted in many Natural Language Processing (NLP) applications such as machine translation~\cite{bahdanau2014neural}, dialogue generation~\cite{li2017adversarial} and image captioning~\cite{fang2015captions}. Previous approaches generally maximize the log-likelihood of ground-truth sentences. However, in theory, this approach suffers from exposure bias~\cite{bengio2015scheduled} due to the inherent discrepancy between the training stage and inference stage. That is to say, the model is trained to generate appropriate succeeding token based on ground truth prefix, which is not available during training.

%The problem of exposure bias is avoid as the generator generate tokens based on previous generated tokens in both training and inference stage.%

Generative Adversarial Networks~\cite{goodfellow2014generative} (GANs) have achieved tremendous success for image generation and received much attention in computer vision. For text generation, however, the performance of GANs is severely limited due to reward sparsity and mode collapse: Reward sparsity prevents the generator from learning when its generated samples can hardly fool the discriminator; while mode collapse leads the generator to only learn the limited patterns from the real data. As a result, both the quality and diversity of generated text samples are seriously affected.

To address the above issues, we propose a novel self-adversarial learning (SAL) paradigm for improving adversarial text generation. In contrast to standard GANs (Figure \ref{fig:sal}(a)) that use a binary classifier as its discriminator to predict whether a sample is real or generated, SAL employs a comparative discriminator which is a pairwise classifier assessing whether the currently generated sample is better than a previous one, as shown in Figure \ref{fig:sal}(b).
During training, SAL rewards the generator when its currently generated sentences are found to be better than previous samples generated by itself. In the early training stage when the quality of generated samples is far below the real data, this self-improvement reward mechanism makes it easier for the generator to receive rewards with informative learning signals, effectively alleviating the reward sparsity issue; while in the late training stage, SAL can prevent a similar sample to the real data from keeping receiving high reward as the self-improvement will become more and more difficult, and therefore help the generator avoid collapsing toward the limited patterns of real data.


%We first propose a comparative discriminator in the spirit of learning by comparison to relieve the reward sparsity problem. The comparative discriminator is a pairwise classifier which simultaneously receives a generated sentence and a reference sentence as input and outputs the comparison results indicating the first sentence is of better, comparable or worse quality than the reference sentence. Standard binary discriminator in GANs receives either generated or real sample and outputs a binary score indicating the probability of the received sample being real. When the a good sentence is generated, the binary discriminator would assign high probability to the sentence being real. However, it is indistinguishable whether the generated sentence is indeed better, comparable, or indeed slightly worse compared with real sentences. The comparative discriminator instead assesses the quality of generated sentences by comparing them with reference sentences. It encodes the inductive bias that a generated sample may be better, as well as indistinguishable, compared with real samples. The comparative discriminator is trained to learn a total order of sample quality, which is more challenging than binary discriminator, thus helps reduce the reward sparsity issue. Based on the comparative discriminator, we modify the conventional adversarial learning paradigm to self-adversarial learning, where the generator is trained in a self-play fashion in addition to competing with the discriminator. In SAL, a generated sample is compared with other samples generated by the generator itself, instead of explicitly or implicitly competing with real samples. In the self-play fashion, the assessment of generated samples is adapted to the current capability of the generator and self-improvement, which may be more informative and stable, is measured. The comparative discriminator could not easily recognize generated sentence as fake and provide zero reward, which mitigates the problem of reward sparsity and may improve the quality of generated samples. For the issue of mode collapse, as the generator has to compete with itself which keeps evolving, it can not merely learn limited patterns which resemble real data and keep fooling the discriminator. The diversity of generated samples is thus enhanced. Moreover, the self-improvement reward scheme and 'tie' option of the comparative discriminator could hopefully reduce the instability of adversarial training.

% change the following paragraph to experimental results.

We comprehensively evaluate the proposed self-adversarial learning paradigm on both synthetic data and real data on text generation benchmark platform~\cite{zhu2018texygen}. We evaluate generation quality based on BLEU statistics and perplexity, generation diversity based on backward BLEU statistics and negat  When compared with previous approaches for adversarial text generation, our model shows a substantial improvement in terms of generation quality based on BLEU statistics and perplexity.   

%Our contributions are three-fold: (i) We propose a comparative discriminator which evaluate the quality of generated samples by pairwise comparison. (ii) We introduce a self-adversarial learning paradigm where generator improves in a self-play fashion. (iii) We evaluate our model comprehensively on text generation benchmark platform~\cite{zhu2018texygen}. The comparative discriminator consistently and significantly outperforms both binary discriminator and recently proposed ranker model~\cite{lin2017adversarial}. Self-adversarial learning further improves both the quality and the diversity of generated samples and enhances the training stability at the same time.
%Moreover, simply combining standard adversarial learning and SAL yields incremental improvements.
